TextHacker: Learning based Hybrid Local Search Algorithm for Text Hard-label Adversarial Attack

Existing textual adversarial attacks usually utilize the gradient or prediction confidence to generate adversarial examples, making it hard to be deployed in real-world applications. To this end, we consider a rarely investigated but more rigorous setting, namely hard-label attack, in which the attacker can only access the prediction label. In particular, we find we can learn the importance of different words via the change on prediction label caused by word substitutions on the adversarial examples. Based on this observation, we propose a novel adversarial attack, termed Text Hard-label attacker (TextHacker). TextHacker randomly perturbs lots of words to craft an adversarial example. Then, TextHacker adopts a hybrid local search algorithm with the estimation of word importance from the attack history to minimize the adversarial perturbation. Extensive evaluations for text classification and textual entailment show that TextHacker significantly outperforms existing hard-label attacks regarding the attack performance as well as adversary quality.

==> body/preliminary.tex <==
% In this section, we formulate the problem and briefly introduce hybrid local search algorithm.

% \subsection{Problem Formulation}
Given the input space $\mathcal{X}$ containing all the input texts and the output space $\mathcal{Y}=\{y_1, y_2, \ldots, y_k\}$, a text classifier $f\colon \mathcal{X} \to \mathcal{Y}$ predicts the label $f(x)$ for any input text $x = \langle w_1, w_2,\ldots,w_n \rangle \in \mathcal{X}$, in which $f(x)$ is expected to be equal to its ground-truth label $y_{true} \in \mathcal{Y}$. % with high probability.
The adversary typically adds an imperceptible perturbation on the input text $x$ to craft a textual adversarial example $x^{adv}$ that misleads classifier $ f$:
\begin{equation*}
f(x^{adv}) \ne f(x) = y_{true}, \quad \mathrm{s.t.} \quad d(x^{adv}, x) < \epsilon,
\label{eq:adv_object}
\end{equation*}
where $d(\cdot, \cdot)$ is a distance metric (\eg the $\ell_p$-norm distance or perturbation rate) that measures the distance between the benign sample and adversarial example, and $ \epsilon$ is a hyper-parameter for the maximum magnitude of perturbation. 
We adopt the perturbation rate as the distance metric:
\begin{equation*}
    d(x^{adv},x) = \frac{1}{n}\sum_{i=1}^n \mathbbm{1}(w_i^{adv} \ne w_i), 
\end{equation*}
where $\mathbbm{1}(\cdot)$ is the indicator function and $w_i \in x$, $w_i^{adv} \in x^{adv}$.
Given a correctly classified text $x$, we could reformulate the adversarial attack as minimizing the perturbation between benign sample and adversarial example while keeping adversarial:
% the adversarial attack could be formulated as:
% we could formulate the objective function for the attack as follows:
\begin{equation}
    \argmin_{x^{adv}} d(x^{adv},x) \quad \mathrm{s.t.} \quad f(x^{adv}) \ne f(x). \label{eq:our_object}
\end{equation} 

In this work, we propose a novel hard-label attack, named \name, to craft textual adversarial examples by only accessing the prediction label $f(x)$ for any input sample $x$.  

==> png/ablation_iteration.tex <==

\begin{figure}[tb]
\centering
\includegraphics[width=0.45\textwidth]{png/pdf/ablation_iteration.pdf}
\caption{Ablation study for various maximum number of substitution $T_s$ on attack success rate and various maximum number of generation $T_g$ on perturbation rate on BERT using IMDB dataset.
}
\label{fig:ablation_iteration}
\end{figure}

==> png/attention_3.tex <==
% \begin{figure*}[t]

% \begin{subfigure}{.49\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{png/pdf/weight_table_2.pdf}
%     \caption{Weight Table.}
%     \label{fig:attention_table:weight_table_2}
% \end{subfigure}%
% \hspace{0.2cm}
% \begin{subfigure}{.49\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{png/pdf/attention_table_2.pdf}
%     \caption{Attention Table.}
%     \label{fig:attention_table:attention_table_2}
% \end{subfigure}%

% \caption{The visualization of the weight table in our \name (a) and attention table obtained by the confidence (b),  which represents the word importance of the candidate words of the nouns, verbs, adjectives and adverbs in the original text of Table~\ref{tab:attention_example_2}. The original words are highlighted in \origWord{Cyan}, with each row representing the candidate words for this word. The darker the color of the word, the better for generating adversarial examples, and vice versa.}
% \label{fig:attention_table_2}
% \end{figure*}


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{png/pdf/weight_table_visualization_3.pdf}
\vspace{-0.7cm}
\caption{The visualization of the weight table in our \name and attention table,  representing the word importance of the nouns, verbs, adjectives, adverbs, and their candidate words in the original text. The original words are highlighted in \origWord{Cyan}, with each row representing the candidate words of this word. The substituted words are highlighted in \Red{Red} and are marked with stars. The darker the color of the word, the more important it is.
}
% \vspace{0.2cm}
\label{fig:attention_table_3}
\end{figure*}

==> png/attention_4.tex <==
% \begin{figure*}[t]

% \begin{subfigure}{.49\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{png/pdf/weight_table_2.pdf}
%     \caption{Weight Table.}
%     \label{fig:attention_table:weight_table_2}
% \end{subfigure}%
% \hspace{0.2cm}
% \begin{subfigure}{.49\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{png/pdf/attention_table_2.pdf}
%     \caption{Attention Table.}
%     \label{fig:attention_table:attention_table_2}
% \end{subfigure}%

% \caption{The visualization of the weight table in our \name (a) and attention table obtained by the confidence (b),  which represents the word importance of the candidate words of the nouns, verbs, adjectives and adverbs in the original text of Table~\ref{tab:attention_example_2}. The original words are highlighted in \origWord{Cyan}, with each row representing the candidate words for this word. The darker the color of the word, the better for generating adversarial examples, and vice versa.}
% \label{fig:attention_table_2}
% \end{figure*}


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{png/pdf/weight_table_visualization_4.pdf}
\vspace{-0.7cm}
\caption{The visualization of the weight table in our \name and attention table,  representing the word importance of the nouns, verbs, adjectives, adverbs, and their candidate words in the original text. The original words are highlighted in \origWord{Cyan}, with each row representing the candidate words of this word. The substituted words are highlighted in \Red{Red} and are marked with stars. The darker the color of the word, the more important it is.
}
% \vspace{0.2cm}
\label{fig:attention_table_4}
\end{figure*}

==> png/single_word_importance.tex <==

\begin{figure}[tb]
\centering
% \setlength{\abovecaptionskip}{0.1cm}
\subfigure[Weight-Table]{
\includegraphics[width=0.17\textwidth]{png/pdf/single_word_importance_lma.pdf}} 
\subfigure[Word Saliency]{
\includegraphics[width=0.17\textwidth]{png/pdf/single_word_importance_saliency.pdf}}
\subfigure{
\includegraphics[width=0.1\textwidth]{png/pdf/single_word_importance_legend.pdf}}
\caption{The word importance of the word \textit{badly} and its candidate words generated by weight-table and word saliency.} 
\label{fig:single_word}  
% \vspace{-0.5cm}
\end{figure}

==> png/word_importance.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{png/pdf/word_importance.pdf}
\caption{The word importance of different words obtained by weight-table and word saliency in a random sampled text on BERT using IMDB dataset.
}
\label{fig:word_importance}
\end{figure}

==> tabs/ablation_component.tex <==
\begin{table}[tb]
\centering
\small

\begin{tabular}{lcccc} %表格7列 全部居中显示
\toprule

{\textbf{Method}} & \textbf{Succ. } & \textbf{Pert. }  & \textbf{Sim. } & \textbf{Gram. } \\

\midrule


Random  &  85.6 & 4.5  & 79.2  & 0.6\\
Memetic  & 85.6 &  5.0 & 80.9  & 0.6\\ 
Weight-table  &  \textbf{86.8} & 4.3 & 80.6 & 0.5 \\ 
\textbf{\name}  & \textbf{86.8} & \textbf{4.1} & \textbf{82.2} & \textbf{0.4}\\ 


\bottomrule
\end{tabular}

\caption{Ablation study on the memetic algorithm and weight-table in \name on BERT using IMDB dataset regarding attack success rate (Succ., \%), perturbation rate (Pert., \%), average semantic similarity (Sim., \%) and grammatical error increase rate (Gram., \%).}
\label{tb:ablation_component}
\end{table}
